Privacy-Preserving Gaze Data Streaming in Immersive Interactive Virtual Reality: Robustness and User Experience

Eye tracking is routinely being incorporated into virtual reality (VR) systems. Prior research has shown that eye tracking data, if exposed, can be used for re-identification attacks. The state of our knowledge about currently existing privacy mechanisms is limited to privacy-utility trade-off curves based on data-centric metrics of utility, such as prediction error, and black-box threat models. We propose that for interactive VR applications, it is essential to consider user-centric notions of utility and a variety of threat models. We develop a methodology to evaluate real-time privacy mechanisms for interactive VR applications that incorporate subjective user experience and task performance metrics. We evaluate selected privacy mechanisms using this methodology and find that re-identification accuracy can be decreased to as low as 14% while maintaining a high usability score and reasonable task performance. Finally, we elucidate three threat scenarios (black-box, black-box with exemplars, and white-box) and assess how well the different privacy mechanisms hold up to these adversarial scenarios. This work advances the state of the art in VR privacy by providing a methodology for end-to-end assessment of the risk of re-identification attacks and potential mitigating solutions.

==> pages/_old/3.1azim-ekyt-performance.tex <==
 In Section \ref{subsection:eye-tracking-as-a-biometric} \Ethan{Cited the 1st version of related works, EKYT is not covered in the new sections}, we pointed out a significant downside of the Eye Know You Too (EKYT) model arising from its development with high-frequency, standardized data from Conventional Eye Trackers (CET) \Ethan{this isn't a downside; EKYT is made for conventional eye trackers.  It just has a different data domain than our use case.}. Compared to CET, VR Eye-Trackers (VRET) work at lower frequencies and rely on less standardized tasks, which calls the model’s effectiveness in VR settings into question \Ethan{This sentence isn't clear, what is "rely on less standardized tasks"?}.

\Ethan{Let's try without acronyms and see how it reads}

To investigate this, we tested the EKYT’s re-identification accuracy using both CET and VRET data. \Ethan{Here, it is not clear why we are doing any of this.  The problem hasn't been introduced.}  We carried out these tests using three datasets: GazeBase (CET), GazeBaseVR (VRET), and a dataset we created, named "Ours" (VRET) \Ethan{Two conditions are name VRET}. We maintained a uniform data frequency of 125HZ to facilitate a fair comparison. \Ethan{Did not say which datasets correspond to CET or VRET}

Our findings are summarized in Table \ref{tab:crossdatasetevaluation}, where we examine the re-identification accuracy of EKYT across CET and VRET datasets.

A breakdown of the results reveals that:
\begin{itemize}
    \item CET-trained EKYT surpassed VRET-trained EKYT, achieving a much higher re-identification rate of 78.44\% as opposed to 38.30\%, \emph{when tested on CET data. \Ethan{These numbers are not in the table}}
    \item CET-trained EKYT and VRET-trained EKYT showed a comparable performance, exhibiting re-identification accuracies of 40.48\% and 42.42\% respectively, \emph{when tested on VRET data}.
\end{itemize}

\Ethan{Seeing this, there are way too many acronyms to keep track of.  We don't need to say \{XYZ\} EKYT every time, we can just say \{XYZ\}}

In conclusion \Ethan{Don't say "in conclusion" in the middle of the paper}, while CET-trained EKYT models perform better than those trained with VRET data when evaluated on CET data, it is noteworthy that both show almost identical re-identification accuracies when tested on VRET data.  \Ethan{Say what this means at a high-level, instead of purely the relation between the numbers}

\begin{table}
\centering

\begin{tabular}{|l|l|ll|} 
\hline
\multirow{2}{*}{Duration (s)} & \multirow{2}{*}{Test Tracker Type} & \multicolumn{2}{c|}{Trained Tracker Type}  \\ 
\cline{3-4}
                              &                            &Conventional   & Constrained                      \\ 
\hline
\multirow{3}{*}{5}            & Conventional                       & 66.09 & 18.04                    \\
                              & Constrained                        & 27.04 & 33.87                    \\
                              & Immersive                       & 23.33 & 27.67                    \\ 
\hline
\rowcolor{gray!20}
10                            & Immersive                       & 18.67 & 21.33                    \\ 
\hline
30                            & Immersive                       & 40.33 & 39.67                    \\ 
\hline
\rowcolor{gray!20}
           & Conventional                        & 90.78 & 58.57                    \\
\rowcolor{gray!20}

60                         & Constrained                        & 49.98 & 55.09                    \\
                              \rowcolor{gray!20}

                              & Immersive                       & 56.00 & 54.33                    \\ 
                              
\hline
90                            & Immersive                       & 68.00 & 65.00                    \\
\hline
\end{tabular}

\caption{The table presents re-identification rates (\%) on models trained and evaluated on CET (GazeBase),  CVR (GazeBaseVR) and IIVR (Ours) operating at 125 HZ.}
\label{tab:crossdatasetevaluation}

\end{table}




==> pages/_old/3definitions.tex <==
\section{Definitions of Concepts}

We evaluate the re-identification threat of gaze data collected in immersive virtual reality (VR).  We first describe the implemented privacy preservation techniques in detail.  We then define two distinct threat scenarios that we anticipate could become realized as eye tracking-enabled VR becomes more prevalent.  We then detail the methodology of our re-identification attacks created to test the risks of the aforementioned threat scenarios.  

\subsection{Privacy Protection Mechanisms}

Our collected gaze streams over a full session can be represented as a time series of gaze angles in spherical coordinates $\theta, \psi$ and their corresponding time stamps $t$: $X = \{(\theta_0, \psi_0, t_0),(\theta_1, \psi_1, t_1), \cdots, (\theta_N, \psi_N, t_N)\}$.  The gaze angles are localized relative to the recorded position of the headset, i.e. head pose, thus are constrained roughly to the human field of view.  As our privacy mechanisms are implemented in real-time, the operations are applied on the frame which the gaze is sampled, except in the case of temporal downsampling, which is conditioned on prior frames.

We implement three privacy protection mechanisms proposed by \cite{david-john_privacy-preserving_2021}: additive Gaussian noise, temporal downsampling, and spatial downsampling.  We also introduce weighted average smoothing as a novel mechanism.

\subsubsection{Gaussian Noise}

Gaussian noise is sampled independently for the $\theta, \psi$ gaze angles for every frame.  We use the standard deviation of the noise sample $\sigma$ to control the privacy-utility trade-off provided by the method, yielding the following per-frame operation: $X_n = (\theta + x \sim \mathcal{N}(0, \sigma), \psi + y \sim \mathcal{N}(0, \sigma), t)$.  

\subsubsection{Temporal Downsampling}

Temporal downsampling effectively lowers the sampling rate of a stream of data by a factor $K$.  Data entries with indices where $K$ is not a factor are removed from the data stream, yielding a stream with $N/K$ total entries after downsampling.  

A real-time application may expect a gaze vector at all frames.  Thus, we preserve the original data format by simply copying the gaze directions from the prior time step on frames that would traditionally be removed.  Given a downsampling factor $K$, 

$X_n = \left\{ 
  \begin{array}{ c l }
    (\theta, \psi, t)               & \quad \textrm{if } n \mathbin{\%} K = 0 \\
    (\theta_{n-1}, \psi_{n-1}, t)   & \quad \textrm{otherwise}
  \end{array}
\right.$

\subsubsection{Spatial Downsampling}

Spatial downsampling consists of lowering the spatial resolution of the gaze data, e.g. multiple nearby full-resolution points would be mapped to a single down-sampled point, lowering the spatial fidelity.  To apply spatial downsampling to continuous gaze angles, we first map the angles into a set of discrete points large enough to preserve data quality, choosing 2160 points to cover a $180\degree$ field of view.  We achieve spatial downsampling by remapping the gaze angles into a smaller domain equal to the reference domain divided by $L$.  We map the $\theta, \psi$ angles into the discrete domain of $M = 2160 / L$, providing a step size of $\delta = \frac{180\degree}{M}$.  This yields the following per-frame operation: $X_n = (\lfloor \theta / \delta \rfloor \cdot \delta, \lfloor \psi / \delta \rfloor \cdot \delta, t)$. 

\subsubsection{Smoothing}

We introduce a smoothing operation as a novel privacy protection mechanism.  Smoothing streamed gaze data can remove identifiable features without displacing gaze samples in a jarring way as the above mechanisms can.  Because of this, we hypothesize that users will be most accepting of smoothing; they can consciously correct for the gaze stream's behavior by fixating at an objects for a second longer, for example.

To operate in real-time, we define the current gaze vector as a weighted average of $B$ preceding (smoothed) samples.  The preceding samples are simply stored in a sliding window that is updated every frame.  Larger window sizes equal a more intense smoothing operation, which is more successful at removing identifying features, but introduces a larger temporal delay between the input and output gaze vectors.  Implementation details are shown in Algorithm~\ref{alg:smoothing}.

\begin{algorithm}[t]
\caption{Weighted average smoothing operation}\label{alg:smoothing}
\begin{algorithmic}
\State $B \gets$ \textit{size of window}
\State \texttt{window} $\gets Queue()$ \Comment{Note this Queue pops at the $0^{th}$ index}
\State $D \gets 0$
\For{$i \gets 1$ to $B$} \Comment{Initializing the window}
    \State \texttt{window}$.add([0, 0])$
    \State $D \gets D + i$
\EndFor 
\While{\textit{application is running}}
    \State $V_{real} \gets$ \textit{current gaze vector}
    \State \texttt{window}$.pop()$ 
    \State \texttt{window}$.add(V_{real})$
    \State $V_{smooth} = (0, 0)$
    \For{$i \gets 1$ to $B$}
        \State $V_{smooth}[0] \gets V[0] + $\texttt{window}$[i][0] * i$
        \State $V_{smooth}[1] \gets V[1] + $\texttt{window}$[i][1] * i$
    \EndFor
    \State $V_{smooth} \gets V_{smooth} / D$ 
\EndWhile
\end{algorithmic}
\end{algorithm}







\subsection{Threat Models}

We explore multiple threats to eye tracking re-identification that we expect to become plausible in the next decade as eye tracking technology and VR become more mainstream.  Our threat models are organized according to the information or resources that the adversary has access to; as an adversary becomes more informed of the privatization mechanism, they become increasingly able to counteract the privacy efforts.  Additionally, we provide an example scenario for each of these cases.

In all cases, we make the assumption that the adversary's goal is to obtain the identity of an acquired query gaze stream.  It could be that there is sensitive information connected to either the query gaze stream or existing dataset records, and that a successful attack would link the user's identity or quasi-identifier(s) to the sensitive information.  These sensitive attributes could be concrete records, such as health information or group membership, or could be behavioral notions embedded within in the actual gaze stream \todo{find a cite to extracting sensitive info from eye tracking data}.  Alternatively, the adversary could simply link context from the source application to the found identity for non-consented targeted advertisements or to learn group membership.

\Ethan{I read that black-box and white-box are non-inclusive language, so switching with the recommended alternate terms}
\subsubsection{Opaque Mechanism}

In this scenario, an adversary has acquired a privatized gaze stream but has no knowledge regarding the mechanism applied.  The adversary can attempt to query the privatized record against non-privatized records sourced from elsewhere, such as public datasets.  Before querying, it is possible for the adversary to perform a filtering operation in an attempt to render the privacy mechanism ineffective~\cite{papadimitriou_time_2007}, such as wavelet denoising.

\begin{indentparagraph}
    \textit{A malicious VR gaming application (the adversary) records eye tracking data that has been securely privatized by a user's VR hardware.  By enabling the posting of high scores to social media, the adversary learns the user's identity.  The adversary can then query against released datasets with associated medical diagnosis (autism, alzheimer's, depression, etc.), attempting to verify the user's membership in the dataset.  If successful, the adversary has a platform to perform fraud or blackmail.}
\end{indentparagraph}

\subsubsection{Opaque Mechanism with Exemplars}

Similar to the above scenario, the adversary does not have knowledge to the implementation of the mechanism applied.  However, the adversary has access to a large number of privatized records, possibly paired with a number of non-privatized records.  From here, the adversary could attempt to approximate the mechanism, or perform regression analysis to attempt to learn an inverse function of the mechanism.

\begin{indentparagraph}
    \textit{An adversary has a new VR headset which only releases privatized gaze data streams and an older model which releases raw gaze vectors.  They recruit a number of users to perform the same tasks while wearing both headsets.  When they have a sufficient amount of data, they model a function to invert the privacy mechanism, increasing the chance of re-identification.  From this point on, they can apply that function to other records collected through the same hardware.}
\end{indentparagraph}

% \subsubsection{Transparent Mechanism}

% \subsubsection{Adversary Has Access to Raw Datasets}
% \label{sec:threat-scenario-raw-dataset}

% In this scenario, the adversary acquires privatized streamed gaze data from a headset or application that has implemented a privacy mechanism.  The adversary also has access to a reference dataset with clean, non-privatized gaze data.  This dataset could be acquired through VR training data that appears in a company data leak, or be available in public record, such as recorded replays from an online game.  The adversary attempts to link the privatized query data to a non-privatized entry in their dataset in order to derive sensitive information about the user.

% \subsubsection{Adversary Has Access to Privatized Data}

% In this scenario, we make the assumption that the adversary's dataset used to reference has the same privacy mechanism applied as the query entry.  This scenario is most plausible if all tasks similar enough to be compared have been recorded \textit{with} the mechanism.  This would occur if a specific application or platform securely implements a given privacy mechanism internally, so end-user data is only presented with the mechanism in place.  

% Alternatively, if the adversary has insider knowledge to the implementation of the privacy mechanism that is applied to the query gaze stream, they could reproduce that privacy mechanism and apply to a raw dataset procured as explained in Section~\ref{sec:threat-scenario-raw-dataset}.

\subsection{Re-identification Attacks}

We frame our mechanisms' effectiveness at protecting privacy as the ability to prevent against re-identification.  We structure the attack as follows: an adversary has obtained a dataset of recorded gaze data streams $G = \{G_0, G_1, \cdots, G_n\}$ and corresponding identifying labels $l = \{l_0, l_1, \cdots, l_n\}$.  Given a new gaze data stream $G_{unknown}$ procured from another dataset or application, they wish to identify which user the gaze stream belongs to by querying against $G$ and returning the most likely label $l$.  We define the chance of this query successfully returning the correct identity label as the identification accuracy, expressed as a percentage.

To assess the proposed mechansisms' robustness against re-identification attacks, we use Eye Know You Too (EKYT), the current state-of-the-art method for gaze-based user authentication~\cite{lohr_ekyt_2022}.  EKYT is a dense convolutional neural network trained to classify users' eye movements within a training dataset.  The model is input a stream of eye tracking data at a constant length and frequency, and outputs a classification vector for the corresponding identity.  When deployed outside of the training set, the final classification layer is discarded; instead, the final activation layer's D128 embeddings are concatenated across 4 model folds. 
The embeddings of an enrolled user and an unknown gaze source are compared using cosine similarity distance to authenticate users.  

In the authentication task, a threshold is computed at the equal error rate (EER) and is used to authenticate users against their enrollment embeddings.  However, for the task of re-identification we instead match a query embedding against all embeddings in the reference dataset, returning the label of the most similar embedding.  

In our experiments, we designate our query and reference sets as follows: for a given trial, we segment the recorded gaze data stream into 5 second overlapping segments using a 1 second sliding window.  We linearly interpolate to a consistent 125Hz and generate an EKYT embedding for each segment\footnote{We note that linearly upsampling our recorded data frequency may compromise individual saccade behaviors.  However, prior work shows that saccades can be unreliably tracked at frequencies under 250Hz~\cite{andersson_sampling_2010, van_der_geest_recording_2002}.}.  We use embeddings from a trial within $G_{unknown}$ as the query set, and compare against all of a distinct trial from $G$  as the reference set.  We aggregate the predicted labels from each embedding in the query set, considering the most prominent label as the final result of the query.  We repeat this process for all pairs of trials in each of our experiments.

\todo{Azim's section should be around here, discard this.}
EKYT shows real-world feasibility as an authentication model by achieving a 3.66\% EER on only 5 seconds of a reading task.  However, this is on a conventional eye tracker with 1000Hz data.  To test the gap towards real-world feasibility for consumer-grade VR eye tracking, the authors performed a test using 125Hz data with Gaussian noise @ $\sigma = 0.5\degree$ applied to simulate the lesser spatial precision.  With a 5 second authentication window, the EER was equal to 24.57\%; after increasing to a 60 second window, EER was 12.30\%.  We use the authors' official 125Hz models in our experiments.



==> pages/_old/3re-identification.tex <==
\section{Identification in Immersive Interactive VR}

% \noindent\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}

% \textcolor{blue}{
% {\huge Section Outline}
% \begin{itemize}
%     \item First paragraph, restate our use case and goal for the section (we wish to evaluate whether SOTA identification algorithm is capable of identifying users in immersive interactive VR, which has not been tested.  (Reminder, DGaze was tested in Brendan's paper but have terrible ID rate with RBFN).
%     \item Subsection: Dataset.  Include participant details and study methodology
%     \item Subsection: Identification Methodology (Azim's section).
%     \begin{itemize}
%         \item Lightly describe EYKT
%         \item Describe the data domain is is trained on (Gazebase) frequency and nature of tasks (CET).  Note we brought frequency down to 125hz to best match our intended hardware.
%         \item Describe the data we retrained it on (Gazebasevr) frequency and nature of tasks (CVR).
%         \item Our dataset is already defined, but call out that it is immersive interactive (IIVR)
%         \item Describe methodology for our comparison between the two models.  We need to know the variables we are changing and what our re-id metric means.
%     \end{itemize}
%     \item Subsection: Results.  Azim's table.  We want to look at the comparison in performance of the models and the impact that num seconds made on ID rate.  Takeaway is that we will use CVR trained model for experiments moving forward.
% \end{itemize}
% }

% \noindent\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}

On conventional eye trackers at high frequencies, users can be identified at very high accuracies (91.38\% identification rate, 3.66\% equal error rate)~\cite{lohr_eye_2022}.  In VR settings, it is less clear how reliably users can be identified.  An evaluation of 360\textdegree \space VR image and video datasets using a prior identification method~\cite{george_score_2016} yielded identification rates ranging from 9\% to 85\%~\cite{david-john_privacy-preserving_2021}.  The same analysis also evaluated an immersive interactive dataset where users viewed a scene of dynamic animals which moved around~\cite{hu_dgaze_2020}, yielding only a 3\% identification rate.  The level of interactivity and number of degrees of freedom in VR setups could negatively correlate with the potential to be identified in VR~\cite{ugwitz_eye-tracking_2022}.  In this paper, we present an up-to-date evaluation of re-identification risk in immersive interactive VR tasks using the state-of-the-art identification model.

For this analysis, we distinguish eye tracking data sources into three categories.  \textit{Conventional eye tracking} utilizes high quality static sensors at 1000Hz or greater~\cite{griffith_gazebase_2021}, and are highly identifiable~\cite{lohr_eye_2022}.  We distinguish eye movements collected in VR into two categories: \textit{Immersive interactive VR} is collected in a natural way.  Users directly interact with dynamic objects in the virtual scene, and different users experience the scene at their own rate.  This is reflective of consumer applications, such as VR games or dynamic training scenarios.  On the other hand, \textit{constrained VR} is representative of existing experimental setups.  User movements are limited, such as sitting in a chair~\cite{sitzmann_saliency_2018} or placing the head on a chinrest~\cite{lohr_gazebasevr_2023}, and the tasks are standardized such that all users experience the same stimuli at the same rates.  We hypothesize that these static tasks make the re-identification task easier, as users' high-level gaze behaviors are all driven by the same stimuli. 

We identify the risk of identification in immersive interactive VR, which has not been properly explored using state-of-the-art methods.  To achieve this, we first construct a dynamic VR game to serve as a platform for evaluation.  We then present an analysis of the current state-of-the-art architecture trained both on conventional eye tracking data and VR data, evaluating on conventional eye tracking data (GazeBase~\cite{griffith_gazebase_2021}), constrained VR data (GazeBaseVR~\cite{lohr_gazebasevr_2023}), and immersive interactive VR data (our dataset).  We then discuss our results, giving insights to the current risk of identification in consumer VR and the relationship between re-identification potential and the amount of data made available.

\subsection{Data Collection Methodology}
\label{sec:e1-dataset}

We describe the protocol for our collected dataset which serves as a testbed to evaluate identification in immersive interactive VR.

\subsubsection{Participants}

Survey participants were recruited under IRB approved protocol via several communication channels including word of mouth and electronic mailing list advertisements ($N=X$; X\% male, X\% female,X\% other).  Eligible participants required normal or corrected-to-normal vision without the use of eye glasses.  The racial-ethnic distribution is X\% White, X\% Asian, X\% Black or African American, X\% Hispanic/Latino, where X\% of participants report two or more races.  The median age is X years (IQR = X-X).  

\subsubsection{Procedure}

\todo{Figures for each dataset.  These could be formatted to be our teaser figure.}

Participants were debriefed as being employees in a sandwich shop, and were tasked with assembling as many sandwiches as possible in a 90 second timeframe.  Plates of stacked ingredients were organized on the sandwich assembling counter on each side.  In the center of the counter, participants would assemble their sandwiches on an empty plate.  After a sandwich was completed, a small animation would play and the plate would be cleared, allowing participants to begin the next sandwich.  There was a digital timer within participants' main field of view which displayed the amount of time remaining.  

Before beginning the main task, participants were encouraged to practice picking up and assembling ingredients.  In the experiment, participants did not use controllers; instead, grabbing was driven by hand tracking technology to provide a more immersive experience.  Participants underwent 4 trials of the same task and were allowed time to rest between trials.  

As participants performed the tasks, gaze data was collected passively to evaluate the potential of re-identification attacks and to store area of interest (AOI) data.  Each ingredient plate, the assembly plate, and the timer were all AOI regions with fully-covering bounding boxes being used for AOI collision detection.

\subsubsection{Validation}
\label{sec:validation}

Data was collected using the Meta Quest Pro~\cite{meta_quest_pro}.  Before undergoing the experiment, each participant underwent the headset's eye tracking calibration procedure.  Participants gazed directly at spheres which appeared at random points on the screen and gradually shrank until no longer visible.  To validate the accuracy of collected gaze data, participants performed an eye tracking validation task.  Participants faced a $3 \times 3$ checkerboard of red targets situated 2 meters away spanning a $38.58 \degree$ angle vertically and horizontally.  Participants were instructed to gaze directly at the active target, which would become green.  The active target cycled uniformly; each target was active for 2 seconds total, with no downtime until the next dot became active.  We report a spatial accuracy of $\mu = 2.64$, $\sigma = 1.24$, comparable with existing analysis of the Quest Pro~\cite{wei_preliminary_2023}.

\subsection{Evaluation Methodology}
\label{sec:privacy-methodology}

\Ethan{What are opinions on having the subsections be "methodology" and "results"?  I think it is slightly confusing but can't think of an alternative.}
\MJP{I think the new subheadings and org work well. Also I added comments in Code Editor, let me know which you prefer!}
\Ethan{Hi Michael, direct code edits work well with me.  I'll see if I can turn on/off all comments directly through those commands, so I'll stop commenting out individual comments for now so it's easier to communicate}

We evaluate the identification potential of EKYT models trained on conventional eye tracking data (GazeBase~\cite{griffith_gazebase_2021}) and constrained VR data (GazeBaseVR~\cite{lohr_gazebasevr_2023}).  Both models are trained at 125Hz to best match the frequency of our collected data.  We follow the training and testing methodology of Lohr et al.\footnote{\url{https://dataverse.tdl.org/dataset.xhtml?persistentId=doi:10.18738/T8/61ZGZN}}~\cite{lohr_eye_2022}, and present the average rank-1 Identity retrieval rate averaged over all tasks in the dataset.

To our knowledge, there is no existing immersive interactive VR dataset at the scale required to train the EKYT model effectively.  Therefore, we assess the effectiveness of training on constrained VR data and evaluating on immersive interactive VR data, versus using a model solely trained on conventional eye tracking data.

To evaluate the identification potential on our collected data, we define the following protocol.  We first generate embeddings from the raw eye movement data.  Each 90 second trial of the game is separated into 5 second segments sliding over a 1 second interval.  These 5 second segments are linearly interpolated to a constant 125Hz and processed by the EKYT model to create $512D$ feature embeddings $Emb$, which are stored along with labels $L$ for the individuals as records.

We separate records into folds according to the trials of the game.  So, all records corresponding to the first trial exist in the first fold, and so on.  We then compare pair-wise each fold as a distinct query and reference set.  For each individual, all query records are compared with the records in the embedding set.  So, for $N$ individuals and $M$ records per individuals, $Query_n = \{Emb_{n, 1}, Emb_{n, 2},$ ... $Emb_{n, m}\}$ and reference $Ref = \{\hat{Emb}_{n, m} : \forall n \in N, \forall m \in M \}$.  We match the record from the query to the closest reference embedding using cosine similarity as a distance metric and store the associated label. For an individual $n$, the predicted label $L_{p, n}$ is:

\begin{equation}
\begin{gathered}
    L_{p, n} = \argmax_L \left( \sum_m^M L_{z}\right) \\ \text{where} \quad z = \argmin_m \left( \sum_{n'}^N \sum_{m'}^M \left( 1 - \frac{Query_{n, m} \ \cdot \ Ref_{n', m'}}{||Query_{n, m}|| \ ||Ref_{n', m'}||} \right) \right)
\end{gathered}
\end{equation}

We aggregate the returned labels between each query embedding $Query_{n, m}$ and all embeddings in the reference set to determine a final prediction $L_{p, n}$.  If $L_{p, n}$ equals the true label $L_{n}$, the individual has been successfully identified.

The reported metrics are an average over all individuals and all pair-wise combinations of distinct trials, readable as an average identification accuracy over the full dataset, or the likelihood of any individual being successfully identified.

\subsection{Results}

\input{pages/3.table}

Our findings are reported in Table~\ref{tab:tab}.  We report the accuracies between the 2 training and 3 test setups.  We additionally report results varying the duration of each data record.  These results are calculated using the explained methodology but first limiting the amount of data to the first X seconds per data record.

We find that the model trained on conventional eyetracking data performs well when evaluated in the same domain, reaching identification accuracies of 66.09\% and 90.78\% on 5 second and 60 second data records, respectively.  However, the conventional ET model performs much less effectively in when applied to VR, achieving 27.04\%@5s and 49.98\%@60s on constrained VR and 23.33\%@5s and 56.00\%@60s on immersive interactive VR data.  

On the other hand, the constrained VR model favors VR data at a lower duration (18.04\%@5s for conventional, 33.87\%@5s for constrained VR, 27.67\%@5s for immersive interactive VR) but performs roughly equal on all domains at higher duration (58.57\%@60s for conventional, 55.09\%@60s for constrained VR, 54.33\%@60s for immersive interactive VR).  This could be due to GazeBaseVR containing less overall data than GazeBase, or due to VR headsets having lower spatial precision than high quality conventional eye trackers.

We find performance on immersive interactive VR data to be roughly equal between the two models.  While the conventional eye tracking model is trained on a larger dataset, the constrained VR model has closer spatial precision and more similar setup to our data.  For the rest of this paper, we use the constrained VR EKYT model to compute identification accuracies.  





%\input{pages/3.1azim-ekyt-performance}

==> pages/_old/4privacy-mechanisms.tex <==
\section{Privacy Protection}

% \noindent\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}

% \textcolor{blue}{
% {\huge Section Outline}
% \begin{itemize}
%     \item First paragraph, state the need for privacy protection, why sample level data is needed for many applications, real time.
%     \item Subsection to define privacy mechanisms
%     \item methodology on how we applied privacy mechanisms (query is privatized but full reference set is not)
%     \item results
% \end{itemize}
% }

% \noindent\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}

There might be a need to protect users from being identified based on eye tracking movements collected in immersive interactive VR~\cite{miller_personal_2020}.  Eye movements are being incorporated into VR experiences to enable novel forms of interaction, optimizations such as foveated rendering, and to enhance social presence of embodied avatars.  These functionalities will have positive outcomes.  There is substantial risk of untrustworthy applications storing eye movements without users consent to collude with other applications to link identities and build user profiles, or to link identities to sensitive attributes for malicious purposes.  

A potential solution would be to implement privacy operations on the eye movement data securely on VR hardware before releasing data to applications.  Any solution to protect user privacy should be able to operate in real time, as any eye tracking interactions require sample level data at a high frequency in order to operate.  Additionally, the ideal privacy solution should not be constrained by the length of the data entry, because users should not have to trade off their duration in VR with their level of privacy.  Because of this, differential privacy operations~\cite{dwork_differential_2006} may not be suited to the VR use case.

\subsection{Privacy Mechanisms}

Collected gaze streams over a full VR session can be represented as a time series of gaze angles in spherical coordinates $\theta, \psi$ and their corresponding time stamps $t$: $X = \{(\theta_0, \psi_0, t_0),(\theta_1, \psi_1, t_1), \cdots, (\theta_n, \psi_n, t_n)\}$.  The gaze angles are localized relative to the recorded position of the headset, i.e. head pose, thus are constrained roughly to the human field of view.  As our privacy mechanisms are implemented in real-time, the operations are applied directly on the frame which the gaze is sampled.

We implement three privacy protection mechanisms proposed by David-John et al.~\cite{david-john_privacy-preserving_2021}: additive Gaussian noise, temporal downsampling, and spatial downsampling.  We also introduce weighted average smoothing as a novel mechanism.

\subsubsection{Gaussian Noise}

Gaussian noise is sampled independently for the $\theta, \psi$ gaze angles for every frame.  We use the standard deviation of the noise sample $\sigma$ to control the privacy-utility trade-off provided by the method, yielding the following per-frame operation: $X'_n = (\theta_n + x \sim \mathcal{N}(0, \sigma), \psi_n + y \sim \mathcal{N}(0, \sigma), t)$.  

\subsubsection{Temporal Downsampling}

Temporal downsampling effectively lowers the sampling rate of a stream of data by a factor $K$.  Data entries with indices where $K$ is not a factor are removed from the data stream, yielding a stream with $N/K$ total entries after downsampling.  

A real-time application may expect a gaze vector at all frames.  Thus, we preserve the original data format by simply copying the gaze directions from the prior time step on frames that would traditionally be removed.  Given a downsampling factor $K$, 

$X'_n = \left\{ 
  \begin{array}{ c l }
    (\theta_n, \psi_n, t)               & \quad \textrm{if } n \mathbin{\%} K = 0 \\
    (\theta'_{n-1}, \psi'_{n-1}, t)   & \quad \textrm{otherwise}
  \end{array}
\right.$

\subsubsection{Spatial Downsampling}

Spatial downsampling lowers the spatial resolution of the gaze data, e.g. multiple nearby full-resolution points would be mapped to a single down-sampled point, lowering the spatial fidelity.  To apply spatial downsampling to continuous gaze angles, we first map the angles into a set of discrete points large enough to preserve data quality, choosing 2160 points to cover a $180\degree$ field of view.  We achieve spatial downsampling by remapping the gaze angles into a smaller domain equal to the reference domain divided by $L$.  We map the $\theta, \psi$ angles into the discrete domain of $M = 2160 / L$, providing a step size of $\delta = \frac{180\degree}{M}$.  This yields the following per-frame operation: $X'_n = (\lfloor \theta / \delta \rfloor \cdot \delta, \lfloor \psi / \delta \rfloor \cdot \delta, t)$. 

\subsubsection{Smoothing}

We introduce a smoothing operation as a novel privacy protection mechanism.  Smoothing streamed gaze data can remove identifiable features without displacing individual samples in a jarring way as the above mechanisms can.  Because of this, we hypothesize that users will be accepting of smoothing; they can consciously correct for the gaze stream's behavior by fixating at an objects for a second longer, for example.

To operate in real-time, we define the current gaze vector as a weighted average of $B$ preceding (smoothed) samples.  The preceding samples are simply stored in a sliding window that is updated every frame.  The smoothed value is a weighted average of the $B$ values in the window.  Larger window sizes equal a more intense smoothing operation, which is more successful at removing identifying features, but introduces a larger temporal delay between the input and output gaze vectors.  Implementation details are shown in Algorithm~\ref{alg:smoothing}.

\begin{algorithm}[t]
\caption{Weighted average smoothing operation}\label{alg:smoothing}
\begin{algorithmic}
\State $B \gets$ \textit{size of window}
\State \texttt{window} $\gets Queue()$ \Comment{Note that this Queue pops at the $0^{th}$ index}
\State $D \gets 0$
\For{$i \gets 1$ to $B$} \Comment{Initializing the window}
    \State \texttt{window}$.add([0, 0])$
    \State $D \gets D + i$
\EndFor 
\While{\textit{application is running}}
    \State $X \gets$ \textit{current gaze vector}
    \State \texttt{window}$.pop()$ 
    \State \texttt{window}$.add(X)$
    \State $X' = (0, 0)$
    \For{$i \gets 1$ to $B$}
        \State $X'[0] \gets X'[0] + $\texttt{window}$[i][0] * i$
        \State $X'[1] \gets X'[1] + $\texttt{window}$[i][1] * i$
    \EndFor
    \State $X' \gets X' / D$ 
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsection{Evaluation Methodology}

We evaluate the effectiveness of each privacy mechanism using the same immersive interactive VR dataset collected in Section~\ref{sec:e1-dataset}.  

Our re-identification methodology is the same as defined in Section~\ref{sec:privacy-methodology}, with the privacy mechanisms applied directly to the query set.  Before processing the set of trials which make up the query set, a privacy mechanism is applied at a given strength.  The privatized results are then processed and compared to the reference set.  This represents the following threat scenario:  

\begin{indentparagraph}
    \textit{An adversary acquires a privatized data record without knowing the identity, then queries against a dataset of records which have known identities attached.}
\end{indentparagraph}

To provide an approximation of utility, we compute a utility score by measuring AOI intersections before and after privatization.  We calculate the multi-class precision and recall, weighted by each AOI class's prevalence as the true label.  We then calculate an overall F1 score which can be interpreted as the mechanism's ability to preserve original AOI behavior after privatization.  In gaze applications, AOI intersections are key to enabling features such as object selection and button presses, so function as a proxy to data-driven notions of utility.  

\subsection{Results}
\label{sec:e1-results}

We compute identification accuracies for each mechanism at multiple strengths to define a privacy curve and measure against AOI F1 scores to estimate the anticipated utility trade-off.  We measure Gaussian noise up to $\sigma = 20\degree$, spatial downsampling up to $L = 256$, temporal downsampling up to $K = 30$, and smoothing up to $B = 300$.  The privacy/ utility trade-off can be seen in Figure~\ref{fig:e1-pu}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/e1_privacy_utility.png}
    \caption{Identification accuracy (solid lines) and AOI retention (dotted lines) of privacy mechanisms applied at various strengths.  X axes have been scaled to provide roughly the same privacy falloff so that utility can be directly compared.  Vertical lines indicate the chosen "low" and "high" strengths of each mechanism.}
    \label{fig:e1-pu}
\end{figure}

Of the previously proposed mechanisms, additive Gaussian noise and spatial downsampling are effective at providing privacy.  The proposed smoothing mechanism also provides a level of privacy, albeit at a higher trade-off in AOI retention.  We have not found temporal downsampling to be an effective privacy mechanism.  It is likely that the EKYT model analyzes relationships between highly separated data samples; by retaining $N/K$ real samples, the model can still accurately identify users until $K$ reaches a point far beyond usable utility.

We introduced smoothing as a novel mechanism to protect user eye movements.  On our data, smoothing shows potential for privacy protection, with similar levels of privacy attained as Gaussian noise and spatial downsampling.  However, AOI retention is lowest for smoothing on the tested dataset, indicating that an application receiving smoothed data would have less reliable accuracy per-sample than other mechanisms.

==> pages/_old/4study-design.tex <==
\section{Study Design}

\todo{figure of all tasks, maybe teaser figure?}

We create a series of immersive VR tasks that serve as test applications in which streamed eye gaze data enables key functionality.  These tasks are fully \textit{immersive} rather than \textit{static} tasks found in many prior analyses.  Static tasks consist of all participants undergoing the same stimuli and actions, such as following a dot on the screen with their gaze or viewing 360\degree images and videos [cite popular datasets].  We hypothesize that these static tasks make the re-identification task easier, as participants high-level gaze behaviors are all driven by the stimuli, and participants can be thresholded based on low-level behaviors within the stimuli constraints.  In contrast, in immersive VR, participants are able to walk around fully and/or interact with multiple environmental objects in any order, making each user's motions and eye tracking data much less predictable.  While static VR tasks more closely align with traditional eye tracking methodologies, immersive VR is much more representative of gaming and immersive workplace applications, so is critical to explore.

We design multiple VR tasks that incorporate eye tracking in different ways.  We incorporate eye tracking for passive information collection, gaze as a pointer paired with a micro-gesture selection trigger, and gaze as the sole control mode, where selections are determined by dwell time.  To validate collected eye tracking data, we designed a validation procedure to verify that eye tracking data was being recorded accurately.  All VR tasks were created in Unity3D and experiments were ran on the Meta Quest Pro.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/making_burger.png}
    \caption{A participant completing a sandwich in experiment E1.}
    \label{fig:making_burger}
\end{figure}

\subsection{E0: Validating Collected Gaze Data}

Before undergoing data collection for any of the forthcoming experiments, participants underwent the Meta Quest Pro's eye tracking calibration process.  Participants would gaze directly at spheres which appeared at random points on the screen and gradually shrank until no longer visible.  To validate the accuracy of collected gaze data after calibration, we had participants undergo short validation task(s) prior to beginning the main experiments.

Participants would stand and gaze towards a $9 \times 9$ checkerboard of red targets situated 2 meters away and spanning a $38.58 \degree$ angle vertically and horizontally.  To validate the quality of eye tracking data, participants were instructed to gaze directly at the active target (active targets became green for the duration).  Participants were informed that the first dot would become active when they pressed a 3DUI \textit{Begin} button in front of them, and that the active dot would cycle uniformly.  Each dot was active for 2 seconds total, with no downtime until the next dot became active.  

To validate the headset fitting and recognition of hand tracking gestures, participants underwent a similar task.  With the same $9 \times 9$ checkerboard, participants could then see a translucent cursor indicating the headset's forward direction.  Participants were informed to align the cursor to the active point and make a pinching gesture with their left hand; after a short delay the next cursor would become active.  This task additionally primed participants on the use of a micro-gesture as a selection, which was needed in later experiment trials.

Participants underwent one round of gaze validation before beginning experiment E1.  Prior to experiment E2, participants sequentially performed 3 rounds of gaze validation and 3 rounds of headset/gesture validation.

\subsection{E1: Passive Gaze Analysis}

\todo{Where to put demographic information?}

In this task, the gaze data collected was not a factor in the outcome of the task, and was simply used to evaluate the threat of re-identification attacks and to store AOI activations.  This scenario captures the gaze utility of applications where AOI dwell times could be used to record user interest in certain objects/ products or be used as predictors for task performance.  AOI intersections generally enable many downstream processes, such as information pop-ups or object selection, so preserving a high AOI accuracy after privatization is necessary to maintain gaze utility.

Participants were debriefed as being employees in a sandwich shop, and were tasked with assembling as many sandwiches as possible in a 90 second timeframe.  Participants had an array of stacked ingredients to either side of them.  In the center of the counter was an empty plate in which participants would assemble their sandwiches.  There was a digital timer within participants' main field of view which displayed the amount of time remaining.  

Before beginning the experiment, participants were encouraged to practice picking up and assembling ingredients.  In the experiment, participants did not use controllers; instead, grabbing was driven by hand tracking technology to provide a more immersive experience.  Participants underwent 4 trials and were given time to rest between trials.

\todo{Could make a full figure with a lot of subfigures for each of the main experiments}

Each ingredient plate, the assembly plate, and the timer were all AOI regions with fully-covering bounding boxes being used for AOI collision detection \todo{create a figure showing some of the AOIs and their bounding boxes}.  To simulate the effect of applying privacy mechanisms, recorded gaze motions were processed then simulated in the Unity scene to compute a new set of AOIs to be compared against the non-privatized AOIs.

\subsection{E2: Gaze as Primary Control Mode}

In this task, participants played a simple first-person shooter (FPS) game using gaze as the sole control mode.  This scenario captures the gaze utility of applications where gaze vectors are used as a pointer or cursor.  Potential applications range from using gaze as an aiming tool, using gaze to select user interface (UI) elements, or having objects in the virtual space react to user gaze, such as non-player characters (NPCs) commenting on fixated objects or key objects being highlighted.  

Participants played a FPS game where they remained in a static position and defeated enemies that periodically spawned and travelled towards the player.  Similar to the Balura task present in GazeBase~\cite{komogortsev_fast_2012, griffith_gazebase_2021}, two types of entities would alternatively spawn in random positions and move towards the player.  \textit{Friendly} entities served as visual distractors and \textit{enemy} entities served as targets; participants were instructed to destroy targets before they could reach the player.  Entities would spawn randomly from 7 uniformly spaced points on a 90$\degree$ arc spaced 6 meters from the player position.  Participants could see a translucent gaze cursor indicating their current gaze direction.  In trials with privacy mechanisms applied, the cursor illustrated the effective gaze direction after privatization.

Each trial of the experiment lasted for $\sim$30 seconds.  30 entities (15 targets and 15 distractors) spawned, increasing in speed from 1 m/s to 5 m/s over the duration of the trial.  By increasing difficulty over the course of the trial we aimed to derive useful performance metrics from participants regardless of skill level.  For each experimental condition, participants would undergo two trials of the game sequentially, followed by the Post-Study System Usability System Usefulness subscale (PSSUQ SYSUSE)~\cite{lewis_pssuq_1992}.

We adopted a within-subjects design; all participants underwent every condition.  Privacy mechanism conditions were either no privacy mechanism applied or Gaussian noise/ spatial downsampling at low and high strengths, in a random order.  The privacy mechanism strengths chosen were derived from the re-identification accuracies found in initial analysis of experiment E1.  The first tested values to achieve below 40\% and 20\% re-identification accuracy were chosen for low and high strengths.  For Gaussian noise, low $\varepsilon=1\degree$ and high $\varepsilon=3\degree$.  For spatial downsampling, low $L=48$ and high $L=144$.

We also investigated two distinct control modes for facilitating the selection of targets.  The first control mode was \textit{fixation-based}; if the gaze vector from the participant's left eye was consistently within a target's bounds for 500 ms, the target was destroyed.  The other control mode was \textit{micro-gesture-based}; participants' gaze vector indicated the selection of targets.  If, for a given frame, the player gaze vector intersected with a target's AOI and the participant performed a pinch gesture with their left hand, the selected target was destroyed.  

Participants underwent all five privacy mechanism conditions in random order with a fixed control mode, then all privacy conditions again in random order with the remaining control mode.  To mitigate an order-effects bias, the order of control mode was counterbalanced among participants.  

==> pages/_old/5.1choice-of-model.tex <==
\subsection{Evaluation Model}
    % In Section \ref{subsection:eye-tracking-as-a-biometric}, we highlighted a major limitation of the Eye Know You Too (EKYT) model. The model was developed using the high-frequency, standardized data recorded with Traditional Eye-Trackers (CET). In contrast, VR Eye-Trackers (VRET) operate at lower frequencies and involve less standardized tasks, raising questions about the model's performance in VR environments.

    % To address these concerns and test the model's re-identification accuracy in different settings, we ran tests to evaluate how the EKYT model performs using VRET and CET data. We used three datasets for this: GazeBase (CET), GazeBaseVR (VRET), and Ours (VRET). To ensure fairness, we standardized the data frequency at 125HZ across all datasets.
    
    % Table \ref{tab:crossdatasetevaluation} displays our findings. There, we evaluated EKYT models trained on GazeBase and GazeBaseVR datasets and evaluated on GazeBase, GazeBaseVR, and our dataset. 

    % Firstly, when evaluation is performed on CET data, models trained on CET datasets clearly outperforms models trained on VRET data with an average re-identification rate of 78.44\% and 38.30\% respectively.  
    
    % The data also suggest that EKYT trained on CET data experience a significant drop in re-identification accuracy when evaluated on VRET datasets with an average re-identification accuracy of 40.48\%. Similarly, the model trained on VRET data experiences a similar level of re-identification accuracy, 42.42\%,  when evaluated on VRET dataset. 
    
    % This observation concludes that EKYT trained on CET data clearly outperforms its VRET counterpart. However, models trained on CET and VRET data experience similar levels of re-identification accuacy when evaluated on VRET data.

    In Section \ref{subsection:eye-tracking-as-a-biometric}, we pointed out a significant downside of the Eye Know You Too (EKYT) model arising from its development with high-frequency, standardized data from Conventional Eye Trackers (CET). Compared to CET, VR Eye-Trackers (VRET) work at lower frequencies and rely on less standardized tasks, which calls the model’s effectiveness in VR settings into question.

    To investigate this, we tested the EKYT’s re-identification accuracy using both CET and VRET data. We carried out these tests using three datasets: GazeBase (CET), GazeBaseVR (VRET), and a dataset we created, named "Ours" (VRET). We maintained a uniform data frequency of 125HZ to facilitate a fair comparison.
    
    Our findings are summarized in Table \ref{tab:crossdatasetevaluation}, where we examine the re-identification accuracy of EKYT across CET and VRET datasets.
    
    A breakdown of the results reveals that:
    \begin{itemize}
        \item CET-trained EKYT surpassed VRET-trained EKYT, achieving a much higher re-identification rate of 78.44\% as opposed to 38.30\%, \emph{when tested on CET data.}
        \item CET-trained EKYT and VRET-trained EKYT showed a comparable performance, exhibiting re-identification accuracies of 40.48\% and 42.42\% respectively, \emph{when tested on VRET data}.
    \end{itemize}
    
    In conclusion, while CET-trained EKYT models perform better than those trained with VRET data when evaluated on CET data, it is noteworthy that both show almost identical re-identification accuracies when tested on VRET data.
    

 
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{|l|l|l|l|} 
    \hline
    \multirow{2}{*}{Test Dataset} & \multirow{2}{*}{Duration (seconds)} & \multicolumn{2}{l|}{EKYT Re-ID Accuracy (\%)}  \\ 
    \cline{3-4}
                                  &                                     & Trained on: GazeBase* & Trained on: GazebaseVR**  \\ 
    \hline
    \hline
    \multirow{2}{*}{GazeBase*}     & 5                                   & 66.09                & 18.04                   \\ 
    \cline{2-4}
                                  & 60                                  & 90.78                & 58.57                   \\ 
    \hline
    \multirow{2}{*}{GazeBaseVR**}   & 5                                   & 27.04                & 33.87                   \\ 
    \cline{2-4}
                                  & 60                                  & 49.98                & 55.09                   \\ 
    \hline
    \multirow{5}{*}{Ours**}         & 5                                   & 23.33                & 27.67                   \\ 
    \cline{2-4}
                                  & 10                                  & 18.67                & 21.33                   \\ 
    \cline{2-4}
                                  & 30                                  & 40.33                & 39.67                   \\ 
    \cline{2-4}
                                  & 60                                  & 56.00                & 54.33                   \\ 
    \cline{2-4}
                                  & 90                                  & 68.00                & 65.00                   \\
    \hline
    \end{tabular}
    }
    \caption{The presented datasets operate at a frequency of 125 Hz. Datasets labeled with a single asterisk (*) represent CET datasets, while those marked with two asterisks (**) represent VRET datasets. The data is organized into four columns, which denote the following: (1) the training set, (2) the testing set, (3) the setup time duration for each data entry, used for querying and referencing each individual, and (4) the re-identification accuracy achieved for each setup }
    \label{tab:crossdatasetevaluation}
\end{table}

     

    

    

    

==> pages/_old/5evaluation.tex <==
\section{Evaluation}

In this section, we provide any additionally relevant detail for evaluating the privacy-utility trade-off for each VR task.  We present the effect of each privacy mechanism and its impact both on re-identification accuracy and each experiment's notion of user utility.

\input{pages/5.1choice-of-model}

\subsection{E0: Validating Collected Gaze Data}

We validate the accuracy of recorded gaze data streams by comparing angular angle between the gaze vector and the center of the active dot.  The median second is processed for each dot to isolate fixations and discard the transitions between dots.  In the gaze validation tasks, we discard the first node from analysis as it was not clear to participants which node would become active.  

We report $2.659\degree \pm 2.121$ validation error for the single gaze validation trial before E1.  Across three repeated trials before E2, we report $2.82\degree \pm 3.095$ for gaze validation and $1.622\degree \pm 1.841$ offset for the headset/ gesture validation, measuring from the point at which the gesture was released.

\subsection{E1: Area-of-Interest Activations}
\label{sec:e1_analysis}

We evaluate the possibility of a successful re-identification attack by considering distinct trials as query and reference gaze data streams.  The results reported are an aggregation of all pairs of trials, e.g. \{trial 1 as query, trial 2 as reference\}, \{trial 1, trial 3\}, \{1, 4\}, \{2, 1\} and so on.

\subsection{E2: Gaze-as-a-Pointer}

\todo{Write about gaze shooter game.}

\subsection{E3: Gaze-as-a-Control-Mode}

\todo{Write about sandwich with gaze (or replacement).}


==> pages/_old/azim-related-work.tex <==
\section{Related Work (Azim)}

\subsection{Eye Movement Identification}

Eye movement is a desirable modality for biometric identification applications, characterized by its uniqueness and persistence \cite{griffith_gazebase_2021}. 
Eye movements are recognized as a form of behavioral biometrics\cite{holland_2011} %\Ethan{replace with behavioral biometric + reference}, 
capable of revealing sensitive details about an individual, including their age, sexual orientation, and personality traits, as referenced in several studies \cite{zhang_how_2018, renaud2002measuring, berkovsky2019detecting} 
% \Ethan{This should be said first in 2.1}.
Building on this premise, eye movements have been researched in a biometric context, with numerous papers proposing statistical \cite{yoon2014gaze, galdi2013new, cantoni2015gant} and deep learning approaches \cite{lohr_eye_know_you_2022, lohr_ekyt_2022}. 

%\Ethan{These cited papers are datasets, not papers that look at biometrics}.
% \textcolor{orange}{AI: Added papers that focused specifally on gaze as a biometric} 

Numerous datasets have been compiled using conventional or virtual reality eye trackers, with frequencies up to 1000 Hz and 250 Hz respectively. Conventional trackers were used in \cite{griffith_gazebase_2021, sbm_dataset, aziz2022synchroneyes, borji2015cat2000}, while virtual reality trackers were employed in \cite{lohr_gazebasevr_2023, hu_dgaze_2020, agtzidis2019360, sitzmann2018saliency, xu2018gaze, david-john_privacy-preserving_2021}. Notably, GazeBase and GazeBaseVR have the highest participant counts among these, with 322 and 407 respectively.% and complemented by the datasets such as GazeBase\cite{griffith_gazebase_2021}, GazeBaseVR \cite{lohr_gazebasevr_2023}, VREM-R1 \cite{vrem_r1_dataset}, SBA-ST \cite{sbm_dataset}, MPIIDPEye\cite{steil_privacy-aware_2019} VR-Saliency\cite{sitzmann2018saliency}, and 360\_em\cite{agtzidis2019360}.


% Goal: Introduce EKYT as the current state of the art model. Describe its architecture briefly maybe. Describe that it achieve re-identification results of 90\% and EER of 0.38\%. Then introduce Brendands model that achieve the highest identification on streaming data. Note that he achieved bad re-identification rates on Dgaze, a dataset that had an unconstrained VR experience. This dataset differs in that participants moved through two 3D rendered virtual scenes using a controller for teleportation for several minutes at a time, instead of viewing many 360° scenes from a fixed viewpoint. This had a huge impact on the re-identification rates and thus requires a consdirable consideration

The current state-of-the-art model, Eye Know You Too\cite{lohr_ekyt_2022}, presents a re-identification rate of 90.56\% when evaluated on non-streaming data. However, in a streaming context, the model proposed by David-John \textit{et al.}\cite{david-john_privacy-preserving_2021} holds the status. The model achieves a re-identification rate of 85\% when evaluated on 360° scenes viewed from a single viewpoint. However, the same model achieves a re-identification rate of 3\% when evaluated on 3D rendered virtual scenes under free-viewing conditions and high levels of immersion. The observed discrepancy in re-identification rates suggests that the level of immersion and free-viewing conditions affect these rates.



%       %\Ethan{Do not write conventional versus VR as early vs new, they are different domains and VR research does not make conventional research obsolete.}\textcolor{orange}{AI: Removed the notion of old datasets.}  
% Conventional eye trackers capture eye movements at a high sampling rate, reaching up to 1000 Hz, within constrained environments where users align their heads using a chin or headrest at a predetermined distance and angle from a computer monitor.
% Datasets such as GazeBase and SBA-ST were obtained using these devices. The elevated sampling rate and controlled conditions have led researchers to report high re-identification performance when assessing methods with these datasets\cite{lohr_ekyt_2022}. 
%\Ethan{again, this is a dataset citation, not a biometric ID paper}.
% \textcolor{orange}{AI: Fixed to EKYT citation.} 
% Virtual reality eye-trackers function at a lower sampling frequency, recording eye movements at up to 250Hz. The environment can be either constrained, requiring a use of chin/headrest, or unconstrained, where such accessories are not used. 

% During the development of these datasets, two primary devices were employed by researchers to track eye movements: conventional and virtual reality eye trackers. Conventional devices capture eye movements at rates as high as 1000 Hz, working within environments where users secure their heads using chin or headrests at defined distances and angles relative to a monitor. Virtual reality eye trackers, however, capture at a maximum rate of 250Hz and can operate in either constrained settings, using chin or headrests, or immersive ones, where such accessories are not required.

% Datasets developed with conventional trackers include GazeBase and SBA-ST. The high frequency of conventional eye trackers lead to re-identification performance of x\% andc EER rate of 0.38\%\cite{lohr_ekyt_2022}. Conversely, in the realm of virtual reality eye tracking, datasets from constrained settings comprise GazeBaseVR, VREM-R1, and MPIIDPEye, while those from immersive settings feature VR-Saliency and 360\_em. To date, no research has evaluated re-identification performance in either settings for virtual reality trackers.




% Datasets like GazeBaseVR, VREM-R1, and MPIIDPEye fall under the category of constrained datasets. On the other hand, VR-Saliency and 360\_em are representative examples of unconstrained datasets. Currently, there is a lack of research that would have reported identification rates within either constrained or unconstrained environments \textcolor{orange}{AI: Is this correct?.} . However, these trackers  attracted considerable attention from commercial companies. This is evident in their recent launches of consumer-level devices with eye-tracking capabilities.
% \footnote{Magic Leap 1~\cite{magic_leap_1} in 2018, Vive Pro Eye~\cite{vive_pro_eye} in 2019, HoloLens 2~\cite{hololens_2} in 2019, Vive Focus 3~\cite{vive_focus_3} in 2021, Magic Leap 2~\cite{magic_leap_2} in 2022, and Meta Quest Pro~\cite{meta_quest_pro} in 2023.  The Apple Vision Pro~\cite{apple_vision_pro} }

% \Ethan{these are all VR headsets but it isn't specified.  Go back to the way they had been listed as a footnote with each device + release year + citation}\textcolor{orange}{AI: copied the footnote}. 

% While GazeBaseVR and VREM-R1 have advanced the field by utilizing modern eye-tracking technology in virtual reality environments, they exhibit a notable drawback due to the constrained settings employed for data collection. Specifically, requiring participants to position their heads on a chin or headrest fails to replicate real-world conditions, where individuals rarely use such supports. Furthermore, mandating that all participants complete identical tasks does not account for the rich diversity of actions and behaviors exhibited in real-life settings. This deviation from real-world scenarios limits the datasets' applicability. Moving forward, there is a pressing need to develop datasets that facilitate unconstrained user interaction and a broader range of tasks to accurately capture the dynamics of eye movements in real-life settings \Ethan{We have discussed 2 datasets in 3 paragraphs, this is way too much detail for a related works.  There is also no mention of EYK, EYKT, DeepIDLive, RBFN, or statistical methods for authentication.  We want to know what domain they tested on and accuracies/ EERs}.

\subsection{Privatization Method and Utility Trade-Off}
Given the sensitive nature of the information that can be deduced from eye movement data, there has been a concerted effort by researchers to develop mechanisms to anonymize collected eye movement data
% \Ethan{Just say mechanisms to anonymize collected eye movement data} 
. These strategies can be grouped into three categories: 
dataset-level~\cite{liu_differential_privacy_2019}, feature-level~\cite{david-john_for_your_eyes_2022, bozkir_dp_temporal_2021, steil_privacy-aware_2019}, and sample-level~\cite{david-john_privacy-preserving_2023, li_kaleido_2021}. Among these, sample-level strategies stand out to be promising, as they can be used within streaming applications, such as gaze prediction, gaze guidance, and foveated rendering\cite{david-john_privacy-preserving_2023}. 


% \cite{david-john_for_your_eyes_2022, bozkir_dp_temporal_2021, steil_privacy-aware_2019, david-john_privacy-preserving_2023} \Ethan{There are 3 main categories for how eye movement privacy is implemented.  Dataset-level, feature-level, and sample-level.  We want to list references for each category and elaborate a bit on sample level.}. 
% However, it is important to note that these methods have limitations, particularly regarding the length of the data streams they can handle \cite{li_kaleido_2021, steil_privacy-aware_2019}. Over time, if the noise sampling pattern in the data becomes known, it becomes possible to reverse the differential privacy (DP) operations \Ethan{Most of the methods you listed are not a form of differential privacy}, thereby compromising the privacy preservation efforts.

% VR systems are in need of a privacy mechanism that can be applied in real-time on every gaze sample before the data is presented to (potentially unsecure) applications~\cite{selinger_visceral_2023, liebling_privacy_2014}.  Kal$\varepsilon$ido~\cite{li_kaleido_2021} is an initial realization of an online process for eye tracking privacy, implemented on a webcam eye tracking system.  However, Kal$\varepsilon$ido introduces about 8ms of latency on a consumer-grade PC, yet total latency over 15-20ms in VR is known to induce severe dizziness and/or nausea~\cite{abras_latency_2012}.  \cite{david-john_privacy-preserving_2021} introduces multiple privacy mechanisms; these mechanisms were evaluated as offline processes, but can be easily implemented in real-time VR.

% The few existing methods that present privacy solutions to sample-level eye tracking data draw privacy/ utility trade-offs by assessing downstream processes (e.g. saliency maps, area of interest statistics, or activity classification).  However, as we saw in Section~\ref{sec:eye-tracking-virtual-reality}, eye tracking is expected to become a major feature in VR as a control mode and animation driver.  We are the first to consider these use cases in-depth and to define a clear privacy/ utility trade-off with respect to active gaze usage in VR.


In the domain of virtual reality, there exists a pressing need for real-time privacy mechanisms that can be applied to each gaze sample before it is shared with applications, which may not be secure. This issue has been addressed in a number of studies, emphasizing the urgency of the matter \cite{selinger_visceral_2023, liebling_privacy_2014}. An early attempt to provide a solution is seen in the development of Kal$\varepsilon$ido, a system implemented on a webcam eye-tracking setup that works to preserve privacy during online processes \cite{li_kaleido_2021} \Ethan{You introduced this section in the domain of VR, but this is a webcam method.}. Despite being a step in the right direction, it introduces a latency of approximately 8 milliseconds on standard consumer PCs, a drawback considering that a total latency exceeding 15-20 milliseconds in VR environments can induce significant discomfort, including symptoms like severe dizziness and nausea, as documented in previous research \cite{abras_latency_2012}. Another noteworthy contribution is from a study that introduced multiple privacy mechanisms evaluated as offline processes, but with the potential for seamless integration into real-time VR environments \cite{david-john_privacy-preserving_2021} \Ethan{This is our most important reference, we are directly extending this paper, but there are no details here}.

While there are a limited number of methods available currently that offer privacy solutions for sample-level eye-tracking data \Ethan{sample-level data hasn't been defined against the other methods}, they generally establish a balance between privacy and utility by evaluating the impact on downstream processes, such as saliency maps and activity classification. As we discussed in Section~\ref{sec:eye-tracking-virtual-reality} \Ethan{referencing a later section}, eye-tracking is poised to become a fundamental feature in VR, serving critical functions like control mode and animation driving. Our work is pioneering in that we delve deep into these use cases, being the first to clearly delineate the privacy and utility trade-offs pertaining to active gaze usage in VR, thereby establishing a solid foundation for future explorations in this direction."


% \subsection{Eye Tracking in Virtual Reality}
% \label{sec:eye-tracking-virtual-reality}

% Research into the design of gaze contingent virtual systems began more than two decades ago~\cite{danforth_platform_2000, tanriverdi_interacting_2000, duchowski_binocular_2000}.  Multiple consumer-level eye tracking-enabled devices released in recent years\footnote{Magic Leap 1~\cite{magic_leap_1} in 2018, Vive Pro Eye~\cite{vive_pro_eye} in 2019, HoloLens 2~\cite{hololens_2} in 2019, Vive Focus 3~\cite{vive_focus_3} in 2021, Magic Leap 2~\cite{magic_leap_2} in 2022, and Meta Quest Pro~\cite{meta_quest_pro} in 2023.  The Apple Vision Pro~\cite{apple_vision_pro} is set to release in early 2024.} have created a resurgence in interest at the intersection between eye tracking and extended reality (XR).  

% For overviews on eye tracking in VR, we point the reader to \cite{adhanom_eye_tracking_2023} and \cite{clay_eye_tracking_2019}.  We mainly highlight examples of VR systems reliant on eye tracking which are in dire need of privacy solutions.

% \subsubsection{Foveated Rendering}

% Foveated rendering is a rendering technique that mimics the mechanics of the eye to improve performance~\cite{guenter_foveated_2012}.  Foveated rendering can overcome hardware constraints around rendering resolution and lower bandwidth when streaming~\cite{lungaro_gaze-aware_2018}.  While humans see focused objects at high fidelty, objects in the peripheral become increasingly out of focus dependent on where in the peripheral and depth offsets from the focused object.  In VR, the fovea region covers only about 4\% of pixels~\cite{patney_perceptually_2016}; most pixels are therefore wasted computations at full fidelity.  Foveated rendering methods determine the fovea region based on gaze direction, then sparsely sample pixels in the peripheral, vastly reducing the number of rendering computations while achieving perceptually similar results to traditional rendering~\cite{weier_foveated_2016, weier_foveated_2018, kaplanyan_deepfovea_2019}\todo{could find more foveated rendering papers, could list out perceptual results, could group deep learning based methods}.  Foveated rendering requires a continuous stream of gaze vectors, so, as we will see in Section~\ref{sec:eye_tracking_privacy}, current implementations have a significant risk of privacy leakage.

% \subsubsection{Gaze Controllers}

% Eye gaze is a viable interaction mode, either on its own or when paired with other control modes.  There is a need in immersive VR to be able to perform secondary tasks while the hands are occupied with a primary action; eye tracking is a suitable choice~\cite{monterio_hands-free_2021}.  Continuous fixations can be thresholded by dwell time to select objects~\cite{gowases_gaze_2008, atienze_interaction_2016}.  Gaze can be used to point out objects which are selected by button presses or gestures~\cite{piumsomboon_interaction_2017, gowases_gaze_2008}.  The upcoming Apple Vision Pro will support gaze-controlled interfaces paired with pinching gestures~\cite{apple_vision_pro}.

% Gaze vectors have recently been used to predict intent to select an object in the future~\cite{david-john_prediction_2021, hu_dgaze_2020} and to model users' emotional or cognitive state~\cite{hare_player_2023}.\todo{can comb them for further references to put here}.  On desktop PCs, eye tracking is used in games\footnote{\url{https://www.digitaltrends.com/gaming/every-pc-game-with-tobii-eye-tracking-support/}} for gameplay mechanics~\cite{antunes_gameplay_2018} and as an accessibility accommodation~\cite{edughele_assistive_2022, vickers_accessible_2013, de_araujo_disabilities_2020}.  VR is seeing similar use as hardware options become available\footnote{\url{https://www.psfanatic.com/here-are-all-the-psvr2-games-that-use-eye-tracking-in-cool-ways/}}.

% \subsubsection{Social Contexts}

% Recorded gaze can be used to drive eye animations in VR.  More realistic eye movements have been shown in improve the quality of interaction with virtual avatars~\cite{garau_avatar_realism_2003} and to increase perceived presence and avatar realism~\cite{seele_looking_at_you_2017}.  Gaze can enable virtual characters to display trust across multiple expressions and contexts~\cite{normoyle_trust_2013}, and multiple personality traits can be discerned solely through characters' eye motions~\cite{ruhland_personality_2015}.

% \subsection{Eye Tracking Movements as a Biometric}
% \label{subsection:eye-tracking-as-a-biometric}

% It is common knowledge that iris patterns are a strong biometric~\cite{negin_iris_2000}.  Lesser known and more recently discovered, pupil size can be a soft biometric~\cite{nugrahaningshi_pupil_2014} and eye movements can be considered a behavioral biometric~\cite{kasprowski_biometrics_2004}, having unique patterns per individual that can not be consciously controlled.  Current VR hardware allows applications access only to eye movement data for simplicity and as a pre-emptive security measure \Ethan{$\leftarrow$ does that make sense?}.

% As a behavioral biometric, eye movements can effectively authenticate small sets of users but loses accuracy as the number of users becomes large~\cite{friedman_biometric_2022}.  Early methods for eye movement biometrics derive hand-crafted features from gaze streams and classify using statistical methods~\cite{kasprowski_biometrics_2004, schroder_robustness_2020, george_score_level_2016, lohr_eye_movement_2020}, but these have recently been surpassed by deep-learning methods~\cite{makowski_deepeyedentificationlive_2021, lohr_eye_know_you_2022, lohr_ekyt_2022, jia_biometric_2018, peng_eye_opener_2022}.  

% A limitation of these methods is that they test on highly standardized tasks and on data recorded at high frequencies (1kHz), conditions not met in VR applications.  The Eye Know You Too (EKYT) model~\cite{lohr_ekyt_2022}, the current state-of-the-art, considered these constraints and showed feasibility with frequency and spatial precision degraded to be comparable to current VR hardware, achieving a 12.3\% EER on 60 seconds of a reading task.  To our knowledge, there are no published models that train directly on VR eye movements, but an increasing number of VR eye movement datasets~\cite{hu_dgaze_2020, lohr_gazebasevr_2023} signals that VR gaze-based authentication is nearby.

% \subsection{Eye Tracking Privacy}
% \label{sec:eye_tracking_privacy}

% For a comprehensive review of the privacy challenges around eye tracking in VR, we point the reader to \cite{bozkir_survey_2023}.

% A handful of privacy guarantees have been proposed to protect eye tracking data from leaking sensitive features.  These have been applied to protect fixation maps~\cite{liu_differential_privacy_2019}, feature-level data~\cite{david-john_for_your_eyes_2022, bozkir_dp_temporal_2021, steil_privacy-aware_2019}, and sample-level data~\cite{david-john_privacy-preserving_2023}.  These methods preserve some notions of utility, including saliency map generation, document classification, activity classification, and gaze prediction.  The aforementioned methods are a post-process operation on existing datasets.  Additionally, methods based on differential privacy (DP)~\cite{dwork_differential_2006} are constrained by the length of the data streams~\cite{li_kaleido_2021, steil_privacy-aware_2019}; if the noise sampling pattern becomes known over time, the DP operation can be undone.

% VR systems are in need of a privacy mechanism that can be applied in real-time on every gaze sample before the data is presented to (potentially unsecure) applications~\cite{selinger_visceral_2023, liebling_privacy_2014}.  Kal$\varepsilon$ido~\cite{li_kaleido_2021} is an initial realization of an online process for eye tracking privacy, implemented on a webcam eye tracking system.  However, Kal$\varepsilon$ido introduces about 8ms of latency on a consumer-grade PC, yet total latency over 15-20ms in VR is known to induce severe dizziness and/or nausea~\cite{abras_latency_2012}.  \cite{david-john_privacy-preserving_2021} introduces multiple privacy mechanisms; these mechanisms were evaluated as offline processes, but can be easily implemented in real-time VR.

% The few existing methods that present privacy solutions to sample-level eye tracking data draw privacy/ utility trade-offs by assessing downstream processes (e.g. saliency maps, area of interest statistics, or activity classification).  However, as we saw in Section~\ref{sec:eye-tracking-virtual-reality}, eye tracking is expected to become a major feature in VR as a control mode and animation driver.  We are the first to consider these use cases in-depth and to define a clear privacy/ utility trade-off with respect to active gaze usage in VR.


==> pages/_old/related-work-v1.tex <==
\section{Related Work}

\subsection{Eye Tracking in Virtual Reality}
\label{sec:eye-tracking-virtual-reality}

Research into the design of gaze contingent virtual systems began more than two decades ago~\cite{danforth_platform_2000, tanriverdi_interacting_2000, duchowski_binocular_2000}.  Multiple consumer-level eye tracking-enabled devices released in recent years\footnote{Magic Leap 1~\cite{magic_leap_1} in 2018, Vive Pro Eye~\cite{vive_pro_eye} in 2019, HoloLens 2~\cite{hololens_2} in 2019, Vive Focus 3~\cite{vive_focus_3} in 2021, Magic Leap 2~\cite{magic_leap_2} in 2022, and Meta Quest Pro~\cite{meta_quest_pro} in 2023.  The Apple Vision Pro~\cite{apple_vision_pro} is set to release in early 2024.} have created a resurgence in interest at the intersection between eye tracking and extended reality (XR).  

For overviews on eye tracking in VR, we point the reader to \cite{adhanom_eye_tracking_2023} and \cite{clay_eye_tracking_2019}.  We mainly highlight examples of VR systems reliant on eye tracking which are in dire need of privacy solutions.

\subsubsection{Foveated Rendering}

Foveated rendering is a rendering technique that mimics the mechanics of the eye to improve performance~\cite{guenter_foveated_2012}.  Foveated rendering can overcome hardware constraints around rendering resolution and lower bandwidth when streaming~\cite{lungaro_gaze-aware_2018}.  While humans see focused objects at high fidelty, objects in the peripheral become increasingly out of focus dependent on where in the peripheral and depth offsets from the focused object.  In VR, the fovea region covers only about 4\% of pixels~\cite{patney_perceptually_2016}; most pixels are therefore wasted computations at full fidelity.  Foveated rendering methods determine the fovea region based on gaze direction, then sparsely sample pixels in the peripheral, vastly reducing the number of rendering computations while achieving perceptually similar results to traditional rendering~\cite{weier_foveated_2016, weier_foveated_2018, kaplanyan_deepfovea_2019}\todo{could find more foveated rendering papers, could list out perceptual results, could group deep learning based methods}.  Foveated rendering requires a continuous stream of gaze vectors, so, as we will see in Section~\ref{sec:eye_tracking_privacy}, current implementations have a significant risk of privacy leakage.

\subsubsection{Gaze Controllers}

Eye gaze is a viable interaction mode, either on its own or when paired with other control modes.  There is a need in immersive VR to be able to perform secondary tasks while the hands are occupied with a primary action; eye tracking is a suitable choice~\cite{monterio_hands-free_2021}.  Continuous fixations can be thresholded by dwell time to select objects~\cite{gowases_gaze_2008, atienze_interaction_2016}.  Gaze can be used to point out objects which are selected by button presses or gestures~\cite{piumsomboon_interaction_2017, gowases_gaze_2008}.  The upcoming Apple Vision Pro will support gaze-controlled interfaces paired with pinching gestures~\cite{apple_vision_pro}.

Gaze vectors have recently been used to predict intent to select an object in the future~\cite{david-john_prediction_2021, hu_dgaze_2020} and to model users' emotional or cognitive state~\cite{hare_player_2023}.\todo{can comb them for further references to put here}.  On desktop PCs, eye tracking is used in games\footnote{\url{https://www.digitaltrends.com/gaming/every-pc-game-with-tobii-eye-tracking-support/}} for gameplay mechanics~\cite{antunes_gameplay_2018} and as an accessibility accommodation~\cite{edughele_assistive_2022, vickers_accessible_2013, de_araujo_disabilities_2020}.  VR is seeing similar use as hardware options become available\footnote{\url{https://www.psfanatic.com/here-are-all-the-psvr2-games-that-use-eye-tracking-in-cool-ways/}}.

\subsubsection{Social Contexts}

Recorded gaze can be used to drive eye animations in VR.  More realistic eye movements have been shown in improve the quality of interaction with virtual avatars~\cite{garau_avatar_realism_2003} and to increase perceived presence and avatar realism~\cite{seele_looking_at_you_2017}.  Gaze can enable virtual characters to display trust across multiple expressions and contexts~\cite{normoyle_trust_2013}, and multiple personality traits can be discerned solely through characters' eye motions~\cite{ruhland_personality_2015}.

\subsection{Eye Tracking Movements as a Biometric}
\label{subsection:eye-tracking-as-a-biometric}

It is common knowledge that iris patterns are a strong biometric~\cite{negin_iris_2000}.  Lesser known and more recently discovered, pupil size can be a soft biometric~\cite{nugrahaningshi_pupil_2014} and eye movements can be considered a behavioral biometric~\cite{kasprowski_biometrics_2004}, having unique patterns per individual that can not be consciously controlled.  Current VR hardware allows applications access only to eye movement data for simplicity and as a pre-emptive security measure \Ethan{$\leftarrow$ does that make sense?}.

As a behavioral biometric, eye movements can effectively authenticate small sets of users but loses accuracy as the number of users becomes large~\cite{friedman_biometric_2022}.  Early methods for eye movement biometrics derive hand-crafted features from gaze streams and classify using statistical methods~\cite{kasprowski_biometrics_2004, schroder_robustness_2020, george_score_level_2016, lohr_eye_movement_2020}, but these have recently been surpassed by deep-learning methods~\cite{makowski_deepeyedentificationlive_2021, lohr_eye_know_you_2022, lohr_ekyt_2022, jia_biometric_2018, peng_eye_opener_2022}.  

A limitation of these methods is that they test on highly standardized tasks and on data recorded at high frequencies (1kHz), conditions not met in VR applications.  The Eye Know You Too (EKYT) model~\cite{lohr_ekyt_2022}, the current state-of-the-art, considered these constraints and showed feasibility with frequency and spatial precision degraded to be comparable to current VR hardware, achieving a 12.3\% EER on 60 seconds of a reading task.  To our knowledge, there are no published models that train directly on VR eye movements, but an increasing number of VR eye movement datasets~\cite{hu_dgaze_2020, lohr_gazebasevr_2023} signals that VR gaze-based authentication is nearby.

\subsection{Eye Tracking Privacy}
\label{sec:eye_tracking_privacy}

For a comprehensive review of the privacy challenges around eye tracking in VR, we point the reader to \cite{bozkir_survey_2023}.

A handful of privacy guarantees have been proposed to protect eye tracking data from leaking sensitive features.  These have been applied to protect fixation maps~\cite{liu_differential_privacy_2019}, feature-level data~\cite{david-john_for_your_eyes_2022, bozkir_dp_temporal_2021, steil_privacy-aware_2019}, and sample-level data~\cite{david-john_privacy-preserving_2023}.  These methods preserve some notions of utility, including saliency map generation, document classification, activity classification, and gaze prediction.  The aforementioned methods are a post-process operation on existing datasets.  Additionally, methods based on differential privacy (DP)~\cite{dwork_differential_2006} are constrained by the length of the data streams~\cite{li_kaleido_2021, steil_privacy-aware_2019}; if the noise sampling pattern becomes known over time, the DP operation can be undone.

VR systems are in need of a privacy mechanism that can be applied in real-time on every gaze sample before the data is presented to (potentially unsecure) applications~\cite{selinger_visceral_2023, liebling_privacy_2014}.  Kal$\varepsilon$ido~\cite{li_kaleido_2021} is an initial realization of an online process for eye tracking privacy, implemented on a webcam eye tracking system.  However, Kal$\varepsilon$ido introduces about 8ms of latency on a consumer-grade PC, yet total latency over 15-20ms in VR is known to induce severe dizziness and/or nausea~\cite{abras_latency_2012}.  \cite{david-john_privacy-preserving_2021} introduces multiple privacy mechanisms; these mechanisms were evaluated as offline processes, but can be easily implemented in real-time VR.

The few existing methods that present privacy solutions to sample-level eye tracking data draw privacy/ utility trade-offs by assessing downstream processes (e.g. saliency maps, area of interest statistics, or activity classification).  However, as we saw in Section~\ref{sec:eye-tracking-virtual-reality}, eye tracking is expected to become a major feature in VR as a control mode and animation driver.  We are the first to consider these use cases in-depth and to define a clear privacy/ utility trade-off with respect to active gaze usage in VR.
